Energy-Based Residual Latent Transport for Unsupervised Point Cloud Completion

Unsupervised point cloud completion aims to infer the whole geometry of a partial object observation without requiring partial-complete correspondence. Differing from existing deterministic approaches, we advocate generative modeling based unsupervised point cloud completion to explore the missing correspondence. Specifically, we propose a novel framework that performs completion by transforming a partial shape encoding into a complete one using a latent transport module, and it is designed as a latent-space energy-based model (EBM) in an encoder-decoder architecture, aiming to learn a probability distribution conditioned on the partial shape encoding. To train the latent code transport module and the encoder-decoder network jointly, we introduce a residual sampling strategy, where the residual captures the domain gap between partial and complete shape latent spaces. As a generative model-based framework, our method can produce uncertainty maps consistent with human perception, leading to explainable unsupervised point cloud completion. We experimentally show that the proposed method produces high-fidelity completion results, outperforming state-of-the-art models by a significant margin.

==> Unpaired Point Cloud Completion/files/ablation_result.tex <==
\begin{tabular}{l|llll|l}
\hline
Method                & Chair         & Lamp          & Sofa          & Table         & Avg.          \\ \hline
w/o EB transport      & 13.6          & 14.3          & 11.9          & 14.7          & 13.6          \\
w/o residual sampling & 14.4          & 14.6          & 12.2          & 16.6          & 14.5          \\
w/o adversarial loss  & 16.6          & 19.5          & 17.7          & 25.5          & 19.8 \\
Full Model            & \textbf{12.0} & \textbf{12.8} & \textbf{10.3} & \textbf{13.8} & \textbf{12.2} \\  \hline
\end{tabular}

==> Unpaired Point Cloud Completion/files/epn3d_result.tex <==
\begin{tabular}{c|c|cccccccc}
\hline
Method           & Avg. & Plane & Cabinet & Car  & Chair & Lamp & Sofa & Table & Boat \\ \hline
3D-EPN~\cite{dai2017complete}           & 29.1    & 60.0  & 27.0    & 24.0 & 16.0  & 38.0 & 45.0 & 14.0  & 9.0  \\
FoldingNet~\cite{8578127}               & 9.2     & 2.4   & 8.5     & 7.2  & 10.3  & 14.1 & 9.1  & 13.6  & 8.8  \\
PCN~\cite{8491026}                      & 7.6     & 2.0   & 8.0     & 5.0  & 9.0   & 13.0 & 8.0  & 10.0  & 6.0  \\
% TopNet~\cite{8953650}                   & 8.4     & 2.5   & 8.8     & 5.9  & 9.3   & 12.0 & 8.4  & 13.5  & 7.1  \\ 
\hline
Pcl2Pcl~\cite{chen2020pcl2pcl}          & 17.4    & 4.0   & 19.0    & 10.0 & 20.0  & 23.0 & 26.0 & 26.0  & 11.0 \\
C4C.~\cite{wen2021c4c}                  & 14.3    & 3.7   & 12.6    & 8.1  & 14.6  & 18.2 & 26.2 & 22.5  & 8.7  \\
ShapeInv.~\cite{zhang2021unsupervised}   & 23.6     & 4.3   &  20.7   & 11.9 & 20.6  & 25.9 & 54.8 & 38.0   & 12.8  \\
Cai \emph{et al.} ~\cite{Cai_2022_CVPR}             & 13.6     & 3.5   &  12.2   & 9.0 & 12.1  & 17.6 & 26.0 & 19.8   & 8.6  \\
Ours                                    & \textbf{9.4}    & \textbf{2.3}   & \textbf{12.2}    & \textbf{5.8}  & \textbf{12.0}  & \textbf{12.8} & \textbf{10.3} & \textbf{13.8}  & \textbf{5.7}  \\ \hline
\end{tabular}

==> Unpaired Point Cloud Completion/files/scan_result.tex <==
\begin{tabular}{l|l|ll|ll|l}
\hline
\multicolumn{1}{c|}{\multirow{2}{*}{Method}} & \multirow{2}{*}{sup.} & \multicolumn{2}{l|}{ScanNet}       & \multicolumn{2}{l|}{MatterPort3D}  & KITTI \\ \cline{3-7} 
\multicolumn{1}{c|}{}                        &                       & \multicolumn{1}{l|}{Chair} & Table & \multicolumn{1}{l|}{Chair} & Table & Car   \\ \hline
GRNet~\cite{xie2020grnet}                    & yes                   & \multicolumn{1}{l|}{1.6}   & 1.6   & \multicolumn{1}{l|}{1.6}   & 1.5   & 2.2   \\
PoinTr~\cite{Yu_2021_ICCV}                   & yes                   & \multicolumn{1}{l|}{1.7}   & 1.5   & \multicolumn{1}{l|}{1.8}   & 1.3   & 1.9   \\ \hline
C4C.~\cite{wen2021c4c}                       & no                    & \multicolumn{1}{l|}{12.0}  & 31.0  & \multicolumn{1}{l|}{12.0}  & 34.0  & 13.7  \\
ShapeInv.~\cite{zhang2021unsupervised}        & no                    & \multicolumn{1}{l|}{5.0}   & 3.0   & \multicolumn{1}{l|}{5.0}   & 3.0   & 6.0   \\
% *Stru.~\cite{Cai_2022_CVPR}                  & no                    & \multicolumn{1}{l|}{3.2}   & 2.7   & \multicolumn{1}{l|}{3.3}   & 2.7   & 4.2   \\
Ours                                         & no                    & \multicolumn{1}{l|}{4.0}   & 3.0   & \multicolumn{1}{l|}{4.0}   & 3.0   & 7.3   \\ \hline
\end{tabular}
